A Syntax-Guided Edit Decoder for Neural Program Repair

Automated Program Repair (APR) helps improve the efficiency of software development and maintenance. Recent APR techniques use deep learning, particularly the encoder-decoder architecture, to generate patches. Though existing DL-based APR approaches have proposed different encoder architectures, the decoder remains to be the standard one, which generates a sequence of tokens one by one to replace the faulty statement. This decoder has multiple limitations: 1) allowing to generate syntactically incorrect programs, 2) inefficiently representing small edits, and 3) not being able to generate project-specific identifiers. In this paper, we propose Recoder, a syntax-guided edit decoder with placeholder generation. Recoder is novel in multiple aspects: 1) Recoder generates edits rather than modified code, allowing efficient representation of small edits; 2) Recoder is syntax-guided, with the novel provider/decider architecture to ensure the syntactic correctness of the patched program and accurate generation; 3) Recoder generates placeholders that could be instantiated as project-specific identifiers later. We conduct experiments to evaluate Recoder on 395 bugs from Defects4J v1.2 and 420 additional bugs from Defects4J v2.0. Our results show that Recoder repairs 53 bugs on Defects4J v1.2, which achieves 21.4% improvement over the previous state-of-the-art approach for single-hunk bugs (TBar). Importantly, to our knowledge, Recoder is the first DL-based APR approach that has outperformed the traditional APR approaches on this dataset. Furthermore, Recoder also repairs 19 bugs on the additional bugs from Defects4J v2.0, which is 137.5% more than TBar (8 bugs) and 850% more than SimFix (2 bugs). This result suggests that Recoder has better generalizability than existing APR approaches.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> intro2.tex <==
\section{Introduction}
Automated program repair (APR) aims to reduce the bug-fixing effort by generating the patches to aid the developers. Due to the well-known problem of weak test suite~\cite{PatchPlausibility}, even if a patch passes all the tests, the patch still has a high probability to be an incorrect patch. To overcome this problem, existing approaches have used different means to guide the generation of patches. A typical way is to learn from existing software repositories, such as learning patterns from existing patches~\cite{6606626,2018Shaping,DBLP:conf/kbse/JiangRXZ19,10.1145/3293882.3330577,genesis,DBLP:journals/pacmpl/BaderSP019,DBLP:conf/icse/RolimSDPGGSH17}, and using program code to guide the generation of the patches~\cite{xiong-icse17,Long2016,2018Shaping,ELIXIR,L2S-GI18}. 

Deep learning is known as a powerful machine learning approach. Recently, a series of research efforts have attempted to use deep learning (DL) techniques to learn from existing patches for program repair~\citep{8827954,DBLP:journals/corr/abs-1812-07170,9000077,dlfix}. A typical DL-based approach uses the encoder-decoder architecture~\cite{Bahdanau2015NeuralMT} to repair programs: first the encoder encodes the faulty statement as well as any necessary code context into a fixed-length internal representation, and the decoder generates from the internal representation token-by-token a new statement to replace the faulty statement. For example, \citet{DBLP:journals/corr/abs-1812-07170} and \citet{9000077} adopt an existing neural machine translation architecture, NMT, to generate the bug fix; SequenceR~\cite{8827954} uses a sequence-to-sequence neural model with a copy mechanism; DLFix~\citep{dlfix} further encodes the faulty statement as an AST tree rather than a sequence of tokens, and encodes the context of the statement. 

However, despite multiple existing efforts, the DL-based APR approaches have not yet outperformed traditional APR approaches. Since deep learning has outperformed traditional approaches in many domains, in this paper we aim to further improve the performance of DL-based APR to understand whether we could outperform traditional APR using a DL-based approach. We observe that, though existing DL-based APR approaches have proposed different encoder architectures for APR, the decoder architecture remains to be the standard one: generating a sequence of tokens one by one to replace the original faulty program fragment. The use of the standard decoder significantly limits the performance of DL-based APR. Here we highlight two main limitations.

\todo{Consider the names: change, edit, change operation, edit operation}
{\bf (1) Excessively large patch space}. The goal of the decoder is to locate a patch from the patch space. The smaller the patch space, the easier the task. However, viewing a patch as a sequence of tokens unnecessarily enlarge the patch space, making the decoding task difficult. First, this space representation does not consider the constraints in programs, such as the syntax, and includes many syntactically incorrect statements, which can never form a correct patch. 

Second, many patches only modify a small portion of a statement, and re-generating the whole statement leads to an unnecessarily large space. For example, let us consider the patch of Closure-14 defect in the Defects4J benchmark~\cite{defects4j}, as shown in Figure~\ref{fig:pattern-de1}. This patch only changes one token in the statement. If we represent the patch as a new sequence of tokens to replace the old statement, the new sequence of tokens has the length of 13. If the total number of tokens is $n$, a minimum space containing this patch has $n^{13}$ elements. On the other hand, we may represent the patch as a change operation {\tt modify(9, ON\_EX)}, where {\tt 9} is the ID of the token to be replaced and {\tt ON\_EX} is the new token to replace the original token. To generate this patch, a neural network has to make three choices: (1) selecting {\tt modify} from all change operators, (2) selecting {\tt 9} among all location IDs, and (3) selecting {\tt ON\_EX} among all tokens. In other words, under this representation, a minimum space containing this patch has $kmn$ elements, where $k$ is the number of operators and $m$ is the number of tokens in the old statement. Since $k$ and $m$ are much smaller than $n$, representing patches as change operations may significantly reduce the patch space.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Closure-14.pdf}
    \caption{The Patch for Closure-14 in Defects4J }
    \label{fig:pattern-de1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Lang-57.pdf}
    \caption{The Patch for Lang-57 in Defects4J}
    \label{fig:pattern-de2}
\end{figure}


{\bf (2) Insufficiently small patch space}. Unlike natural languages, programming languages often contain locally-defined identifiers. Since it is virtually impossible to include all possibly  identifiers in the patch space, existing DL-based APR approaches only generates identifiers that have frequently appeared in the training set. However, different projects often have different sets of locally-defined identifiers, and considering only the identifiers in the training set may exclude many patches from the patch space. For example, Figure~\ref{fig:pattern-de2} shows the patch for Lang-57 in Defects4J. To generate this patch, we need to generate the identifier ``{\tt availableLocaleSet}'', which is defined in this project and is unlikely to be included in a training set. As a result, existing DL-based approach cannot generate this patch. 

\smallskip
In this paper we propose a novel DL-based APR approach, \techname. Similar to existing approaches, \techname is based on the encoder-decoder architecture. In particular, to address the above two limitations, the decoder of \techname has the following two novel techniques.

\todo{emphasize syntactic correctness}
{\bf (1) Dynamic Syntax-Guided Decoder}.
To ensure the generated code satisfy the syntax, existing DL-based program generation approaches~\cite{treegen,DBLP:conf/acl/YinN17,DBLP:conf/acl/RabinovichSK17,DBLP:conf/aaai/SunZMXLZ19} have used a syntax-guided decoder: in each step, the decoder selects a grammar rule to expand an non-terminal in a partial AST. 
%Repeatedly applying the above procedure for each non-terminal, we can generate a full program from the start symbol. 
We observe that the space of change operations could also be described by a grammar, and thus the idea of syntax-guided decoder may also be applicable. For example, the previous change operation could be described by the grammar: 
\[\begin{array}{rcl}
    {\it Change} &\rightarrow & {\it Insert} \mid {\it Modify} \mid \ldots \\
    {\it Modify} &\rightarrow & {\it Modify}({\it NodeID}, {\it NTerm}) \\
    {\it NodeID} &\rightarrow & \textrm{<An AST Node ID of the faulty statement>} \\
    {\it NTerm} &\rightarrow & \textrm{<The Java non-terminal of {\it NodeID}>} \mid \ldots \\
\end{array}\]

However, different from program generation, the grammar is not a statically fixed one, and may depend on the local context (e.g., the choices of {\it NodeID} depends on the faulty statement) or a previous choice (e.g., the choice of {\it NTerm} depends on the choice of {\it NodeID}). Therefore, the existing syntax-guided decoder which only deals with a statically fixed grammar rule set does not apply. To overcome this problem, we propose dynamic syntax-guided decoder. A dynamic syntax-guided decoder repeatedly visits the unexpanded non-terminal node in an AST, and takes one of the following actions based on the AST node type and the predicted likelihood: (1) select a grammar rule to expand it, (2) choose a node from the faulty statement to modify and constrain {\it NTerm} with the same non-terminal, and (3) copy a subtree from the faulty statement or its context. Each action is performed by an independent neural component. In this way, \techname generates change operations, and ensure the changed program is still syntactically correct. \todo{Consider the alternative: do not introduce all actions here, and add a summary of our approach later}

{\bf (2) Placeholder Generation}. 
To generate the locally-defined identifiers, a direct idea is to add another action that selects an identifier from the local context. However, to perform such an action, a neural component needs to access all user definitions in this project. This is very difficult as no neural component could encode the source code of a whole project. Instead of relying on the neural network to generate locally-defined identifiers, in \techname the neural network simply generates placeholders for such identifiers, and these placeholders are instantiated with all possible local identifiers when applying the change operations. The key insight is that, when considering the constraints in the programming language such as types, the number of choices for replacing a placeholder with local identifiers is small and instantiating the placeholders with all possible choices is manageable.


Our experiment was conducted on two widely used benchmarks: Defects4j v1.2(395 bugs) and Defects4j v2.0(284 bugs). We compared \techname with four state-of-the-art DL-based APR approaches and several pattern-based APR tools. \techname repaired $\bm{52}$ bugs on Defects4j v1.2, which outperforms the existing APR tools by 23.2\% including the pattern-based tools. To our knowledge, this is the first time that neural models achieve better performance than pattern-based tools. Furthermore, \techname also achieves better performance than several state-of-the-art pattern-based APR tools on Defects4j v2.0, which shows the generality of \techname on new defects. To summarize, this paper makes the following contributions:
\begin{itemize}
    \item We propose a syntax driven patch generation model with several novel structural grammars to generate patches based on the tree structure of the code. We design a novel AST-based encoder for the buggy method and two novel neural components for the new proposed grammars.
    \item \techname achieved 23.2\% better performance than the previous start-of-the-art APR tools on Defects4j1.2. \techname is the first DL-based APR that achieves better performance than pattern-based tools on this benchmark.
    \item We show that \techname can fix 2.375 and 19 times more bugs compared with the top two pattern-based APR tools on Defects4j v2.0. This phenomenon shows the overfitting problem of some pattern-based tools. \techname can learn the bug-fixing patterns from the history automatically and has better generality than the pattern-based APR tools. 
\end{itemize}

==> motivation.tex <==
\section{Motivation}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{lang29.pdf}
    \caption{Lang-29 - A bug can not be fixed by pattern-based tools}
    \label{fig:pattern-de}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Closure-14.pdf}
    \caption{Closure-14 - A bug can not be fixed by deep learning based tools}
    \label{fig:pattern-de1}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Lang-57.pdf}
    \caption{Lang-57 - A bug can not be fixed by deep learning based tools}
    \label{fig:pattern-de2}
\end{figure}
As mentioned in Introduction, pattern-based APR tools and deep learning based APR tools have their own disadvantages. For pattern-based APR tools, the patterns used in these approaches are mostly hand-written based on specific projects. When applying to the new projects, they does not work well as the non-include patterns in tools. For example, Lang-29 in Defects4j, can not be fixed by all pattern-based tools, which need a pattern for updating a return type of a function. In this way, programmers have to add a new pattern into the existing tools. However, it is an exhausted task for programmers to write various patterns to cover thousands of the real-world defects. In contrast, the deep learning based approach can learn various patch patterns from thousands of history patches.

For DL-based tools, most of them use machine translation via neural network models with various code abstractions and contexts to generate patches. However, there are some circumstances that a complex expression just need to change a atomic value(a parameter, a operator or a name of method) for repairing. For example, Closure-14 in Defects4j, is difficult for deep learning based approaches to fix. The patch only changes the field of "Branch". The pattern-based tools adopt the mutation based operator to change the field while the deep learning based tools need to generate the complex expression. Thus, deep learning based tools are difficult to handle this kind of patches because the long sequence is hard for neural models to generate. Besides this circumstance, deep learning based tools are also difficult to handle the patches containing out-of-vocabulary tokens. For example, Lang-57 in Defects4j, can not be repaired by any deep learning based tools. The patch replaces the name of method with another one defined in the specific project. Thus, "availableLocalSet" is not in the pre-defined vocabulary because it is a method defined in the user-defined class. 

To address these problems, we propose a general framework for APR to combine the strengths of these two kind of APR tools. This framework contains several stages to repair the given defects. Each stages can be applied to different suitable APR techniques. Thus, we adopt both pattern-based APR approaches and deep learnig based approaches to different stages in this framework. For projects specific defects, we design a stage named Patch Template Completion. We define the outputs of the previous stages as a pattern with several holes not a complete patch. Then, in this stage, several techniques in pattern-based tools can be applied to select the proper method names and class variables in the corresponding project contexts. Furthermore, different from the pattern-based tools, we just define several fix patterns and mutation operators for neural models to select and apply while we do not use heuristic features to apply this patterns. We design a novel sub-model to select the patterns and the position to apply the patterns. Then, we integrate this sub-model with the code generation models which aims to generate patches directly, and the whole model combines the strengths of these two kinds of APR tools.  

==> picture/chart.tex <==
option = {
            title : {
            show:true,
            text: 'Performance of Recoder on Different Size of Dataset',
            x:'center',
            textStyle:{
                fontSize:40, //字体大小
            }
            },
    tooltip: {
        trigger: 'axis',
        axisPointer: {
            type: 'cross',
            crossStyle: {
                color: '#999'
            }
        }
    },
    grid:{
        top:150,
        y2:300
    },
    toolbox: {
        feature: {
            dataView: {show: true, readOnly: false},
            magicType: {show: true, type: ['line', 'bar']},
            restore: {show: true},
            saveAsImage: {show: true}
        }
    },
    legend: {
        data: ['Num', 'Loss'],
        align:'left',
        x:'center',
        y:900,
                    textStyle:{
                fontSize:20, //字体大小
            }
    },
    xAxis: [
        {
            type: 'category',
            data: ['0.25', '0.5', '0.75', '0.85', '0.90', '0.95', '1.00'],
            axisPointer: {
                type: 'shadow',
                
            },
            axisLabel: {
       show: true,
        textStyle: {
          fontSize : 20      //更改坐标轴文字大小
        }
     }
        }
    ],
    yAxis: [
        {
            type: 'value',
            name: 'Num',
            min: 4,
            max: 15,
            interval: 5,
            axisLabel: {
                formatter: '{value} ',
                            textStyle:{
                fontSize:20, //字体大小
            }
            },
            
            
        },
        {
            type: 'value',
            name: 'Loss',
            min: 0.6,
            max: 0.9,
            interval: 0.05,
            axisLabel: {
                formatter: '{value} ',
                            textStyle:{
                fontSize:20, //字体大小
            }
            }
        }
    ],
    series: [
        {
            name: 'Num',
            type: 'bar',
            data: [5, 8, 10, 10, 12, 12, 14],
            itemStyle: {
							normal: {
								label: {
									show: true, //开启显示
									position: 'top', //在上方显示
									textStyle: { //数值样式
										color: 'black',
										fontSize: 24
									}
								}
							}
            }
        },
        {
            name: 'Loss',
            type: 'line',
            yAxisIndex: 1,
            data: [0.87, 0.80, 0.77, 0.72, 0.70, 0.68, 0.67],
                        itemStyle: {
							normal: {
								label: {
									show: true, //开启显示
									position: 'top', //在上方显示
									textStyle: { //数值样式
										color: 'orange',
										fontSize: 24
									}
								}
							}
            }
        }
    ]
};
